DiffusionSeeder: Seeding Motion Optimization with Diffusion for Rapid Motion Planning

Running optimization across many parallel seeds leveraging GPU compute have relaxed the need for a good initialization, but this can fail if the problem is highly non-convex as all seeds could get stuck in local minima. One such setting is collision-free motion optimization for robot manipulation, where optimization converges quickly on easy problems but struggle in obstacle dense environments (e.g., a cluttered cabinet or table). In these situations, graph-based planning algorithms are used to obtain seeds, resulting in significant slowdowns. We propose DiffusionSeeder, a diffusion based approach that generates trajectories to seed motion optimization for rapid robot motion planning. DiffusionSeeder takes the initial depth image observation of the scene and generates high quality, multi-modal trajectories that are then fine-tuned with a few iterations of motion optimization. We integrate DiffusionSeeder to generate the seed trajectories for cuRobo, a GPU-accelerated motion optimization method, which results in 12x speed up on average, and 36x speed up for more complicated problems, while achieving 10% higher success rate in partially observed simulation environments. Our results show the effectiveness of using diverse solutions from a learned diffusion model. Physical experiments on a Franka robot demonstrate the sim2real transfer of DiffusionSeeder to the real robot, with an average success rate of 86% and planning time of 26ms, improving on cuRobo by 51% higher success rate while also being 2.5x faster.

==> response.tex <==
 \onecolumn
\newcommand{\rvo}{ \textcolor{olive}{R-JudU}}
\newcommand{\rvto}{\textcolor{blue}{R-xuWR}}
\newcommand{\rvth}{ \textcolor{pink}{R-MRuk}}

 \noindent We thank all reviewers for their valuable feedback! We appreciate that the reviewers think that \projname{} is \textit{``simple and effective''} and \textit{``a useful and well-executed idea'} [\rvto{}], \textit{``the obtained results are very impressive''}, \textit{``sets a new state-of-the-art for manipulation planning in cluttered scenes from depth images``} and \textit{``is technically sound``}[\rvth{}]. The reviewers also agree that \textit{``the experimental validation is thorough''} [\rvo{}] and that the paper is \textit{``well-written''} [\rvto{}] and \textit{``clear and easy to follow``} [\rvth{}].\\

\noindent Based on the reviewer feedback, we performed the following additional experiments:
\begin{enumerate}
    \item In response to \rvto{}'s concern about the completeness of the baselines, \textbf{we have added the comparison of \projname{} with \bit{} as recommend by \rvto{} in Section~\ref{sec:exp} Table~\ref{tab:depth_res} and Table~\ref{tab:gt_res}}. Results suggest that in both the partial observation and full observation scenarios, \projname{} outperforms \bit{} by a large margin in term of both the success rate and planning time. In addition, the low success rate of \bit{} provides a benchmark for the difficulty of the problems. \textbf{As suggested by \rvto{}, we have also added experiments on \projname{} without \curobo{} in the Appendix Table~\ref{tab:diff_only}}, where the success rate of \projname{} is an order of magnitude higher than that of \mpinet{} and \bit{}, indicating that \projname{} can generate collision free seed trajectories.
    
    \item \rvto{} raises concerns about the effectiveness of the diffusion model in \projname{}. Compared to a feedfoward policy, the advantage of diffusion model comes from the generation of multiple diverse trajectories in one inference pass. \textbf{We added experiments on the performance of \projname{} with \curobo{} with different $N_{trajs}$ in the Appendix Table~\ref{tab:abla_ntraj}.} Results suggest that the success rate of $N_{trajs}=12$ is 1.99x higher than that of $N_{trajs}=1$, showing the benefits of the diffusion model in generating multiple diverse seeds compared to a feedfoward policy which generates one seed. \textbf{Table~\ref{tab:diff_only} in Appendix also suggests that the diffusion model in \projname{} without \curobo{} has an order of magnitude higher success rate compared to a feedforward policy \mpinet{}}, implying that the diffusion model is more effective at generating higher quality seeds for optimizations. In addition, the diffusion model generates the seeds through 5 denoising steps in 6ms, much faster than the feedforward policy (\mpinet{}) which requires more steps to rollout the policy (Table~\ref{tab:depth_res}). 

    \item In response to \rvto{}'s concern about the fairness of the comparison with \curobo{} with $N_{iters}=475$, we clarify $N_{iters}=475$ achieves the best performance for \curobo{} and \textbf{we added \projname{} with $N_{iters}=475$ in Section~\ref{sec:exp}}. As shown in Table~\ref{tab:depth_res}, \projname{}-475 achieves similar success rate to \projname{}-50, which is 10.7\% higher than that of \curobo{}-100. \projname{}-475 also plans 5x faster than \curobo{}-100. 

    \item To address \rvto{}'s concern on that the occlusion challenge is artificially enlarged by using only one depth image, \textbf{we have added experiments on providing more depth images to \projname{} during the inference time in Table~\ref{tab:abla_nvj} in Appendix.} We notice the performance doesn't increase with the number of views, likely because that the model is trained on one depth image. In the future, we hope to train \projname{} on multiple camera views and investigate the performance, to allow more flexible usage of \projname{} when more camera views are available (Section~\ref{discuss}).
    
    

\end{enumerate}

\vspace{5pt}
In addition to the above experiments, we have added comparison with other related work using diffusion-based priors for motion planning [\rvo{},\rvto{}]. We also added clarifications on problem definition, method and experimental setup. The changes are highlighted in \rev{red}. We have reformatted the references to be consistent [\rvth{}].\\

Below, we address various raised questions in detail.

\noindent \textbf{[\rvo{}] Compare the proposed approach with the existing work using diffusion-based priors for motion planning :}\\
Thanks for providing the related works (\cite{janner2022planning,carvalho2024motion,huang2023diffusionbased}) that we overlooked! We have provided a detailed discussion on comparing \projname{} with the three given related works in Section~\ref{sec:rw}. In summary,~\citet{janner2022planning} requires the training of a diffusion model for each new environment as the diffusion model is not conditioned on the environment information, making it impractical for robot motion planning in real life.~\citet{carvalho2024motion} also doesn't provide the environment information to the diffusion model and doesn't generate environment aware trajectory priors. This can be inefficient as the trajectory prior for a shelf environment and a table environment can be very different, resulting an environment agnostic trajectory prior with most of trajectories invalid. In contrast, \projname{} encodes the environment information and generates environment specific trajectories as shown in the supplementary videos. \projname{} generates valid seeds making it more efficient for optimization and generalizes to various unseen scenes.~\cite{huang2023diffusionbased} learns a unified diffusion policy for generation, optimization and planning. For robot motion planning,~\cite{huang2023diffusionbased} utilizes goal oriented planning, which requires multiple policy rollout steps to generate one trajectory, without further optimization of the generated trajectory. Therefore, the trajectory generation is slow and the generated trajectories are suboptimal. \projname{} generates multiple diverse trajectories with 5 denoising steps in 6ms. By providing the generated trajectories to \curobo{}, the final trajectory is optimized to minimize the cost. \\

\noindent \textbf{[\rvo{}] Why the authors did not train on all the scenes together?}\\
\projname{} is trained on all 3M training scenes. Since the scene information is passed to \projname{} as the conditioning, \projname{} works on different environments and generalizes well to real environments. We don't need to train a different model for each scene as in~\cite{janner2022planning}. \\

\noindent \textbf{[\rvo{}] The true generalization ability is something that can be seen based on cross-domain performance.}\\
\projname{} is trained on simulation scenes only but generalizes to real world scenes, as shown in Table~\ref{tab:real_res}. We hope the high success rate of \projname{} on the real world scenes, which are very different from the training scenes, can indicate the ability of \projname{} to generalize.\\

\noindent \textbf{[\rvo{}]Is there a reason that the Diffusion learning pipeline and the Trajectory Optimization are decoupled? }\\
The training objective of the diffusion model is to generate the ground truth trajectories from the noisy trajectory conditioned on the task and environment information. Since the ground truth trajectories are generated by \curobo{} which minimizes the trajectory optimization cost, the diffusion model implicitly minimizes the trajectory optimization cost via the mean squared error with the ground truth trajectory, alleviating the need to provide explicit trajectory optimization cost into the loss.\\

\noindent \textbf{[\rvto{}] Clarification on the definition of ``hard problems" }\\
As suggested by the reviewer, we added the clarification on the definition of ``hard problems" in Figure.~\ref{splash} caption, where ``hard problems" are defined as problems that cannot be solved by using a linear interpolated trajectory for \curobo{}. We also added the baseline \bit{} to provide a benchmark for the hardness of the problems in Section~\ref{sec:exp} Table~\ref{tab:depth_res} and Table~\ref{tab:gt_res}. The low success rate of \bit{} shows the difficulty of the problems.\\

\noindent \textbf{[\rvto{}] Is the occlusion challenge artificially enlarged by restraining the use of one camera?}\\
In most real robot applications, only one or two cameras are set up because setting up multiple cameras requires careful extrinsic calibration and also increases computational costs. Therefore, we mimic the practical real world robot motion planning setup by providing one depth image to \projname{}. However, \projname{} can take in multiple camera views by design. We have added experiments in Table~\ref{tab:abla_nvj} in Appendix on providing more depth images to \projname{} at the inference time, despite the model is trained on one depth image. In the future, we hope to release the checkpoint of \projname{} trained on multiple camera views, allowing more flexible usage of \projname{} when more camera views are available (Section~\ref{discuss}). \\




\noindent \textbf{[\rvto{}] How $N_{iters} = 475$ is selected for \curobo{}. $N_{iters} = 475$ is very likely bad for \curobo{} performance, as it would overoptimize for the partial information (given the fact that it gets 93\% success with $N_iter=1$ once given full information)}\\
We clarify that $N_{iters} = 475$ is shown to achieve the highest success rate for \curobo{}. We have included the clarification in Section~\ref{sssec:curobo} and added a detailed discussion of why $N_{iters}$ for \curobo{} is much higher than that of \projname{} in Section~\ref{sssec:niter}. In short, the initial trajectories of \curobo{} is less optimal, requiring more optimization steps to avoid collision with the partially observed environments and to minimize the cost. 

\noindent We are not sure which 93\% the reviewer is referring to. We assume the reviewer is referring to the 87\% success rate of \curobo{} with \textbf{$N_{atp}=1$} provided the ground truth mesh, which is conducted with $N_{iters} = 475$ and with maximum number of attempts $N_{atp}=1$. The reviewer raises a valid concern that the optimization may over optimize for the partial information. We believe this is not the case as shown in Table~\ref{tab:depth_res}, where the performance of \projname{} with \curobo{} doesn't decrease with increasing $N_{iters}$. If \curobo{} is over optimizing for the partial information, we should expect a performance drop for \projname{} with \curobo{} as well.\\



\noindent \textbf{[\rvto{}] Discussion on the implicit scene completion ability of \projname{} }\\
We agree with the reviewer that collecting training trajectories generated on ground-truth meshes contributes to the implicit scene completion ability of \projname{}. We updated the discussion in Section~\ref{sssec:niter} to reflect this. In addition, since \projname{} sees different views of the same scene during the training, we believe this also contributes to the implicit scene completion of \projname{}. For example, \projname{} sees the left view of a shelf environment and recognizes is as shelf environment. \projname{} can infer the occluded part of the environment as it has seen the other views of the environment.\\

\noindent \textbf{[\rvto{}] The sampling process of training queries is confusing. So all start and goal pairs lie inside the same bounding box of 0.3m? }\\
Each problem in the training dataset from \mpinet{} represents a different configuration of the environment and different start and goal poses for the robot. We take each problem in the dataset and generate new problems by sampling within 0.3m of the original start and goal poses \textbf{respectively}. The start and goal poses of newly sampled problems are \textbf{not} all within the same bounding box of 0.3m. Aggregating across the full dataset, the start and goal poses will cover the full workspace of the robot.\\




\noindent \textbf{[\rvto{}] Training of DDPM: why can the time step k be randomly sampled? Clarifications on DDIM inference. }\\
We have added background on DDPM in Section~\ref{ssec:train} and DDIM in Section~\ref{ssec:infer}. In short, the training objective of DDPM is calculated over the expectation of each time step. To estimate the expectation, we sample different time steps during training.\\

\noindent \textbf{[\rvto{}] Clarifications on image sampling, trajectory length and trajectory normalization.}\\
The 4 depth images are randomly sampled from the valid images (Section~\ref{ssec:env_ren}). The trajectory length is defined as the number of waypoints (Section~\ref{ssec:prob_gen}) and the trajectories are normalized by diving over the joint mechanical limit (Section~\ref{ssec:train}). \\

\noindent \textbf{[\rvth{}] The proposed learning architecture mimics other related diffusion models and offers no new insights that might apply to other areas beyond manipulation planning.}\\
We appreciate that the reviewer thinks ``the obtained results are very impressive" and ``the work sets a new state-of-the-art for manipulation planning in cluttered scenes from depth images"!
While the idea of learning initial seeds for motion planning optimization has been studied, we hope this paper can provide the robotic community with a rapid and practical off-the-shelf motion planning pipeline that works with partial observations. We have added some discussions (Section~\ref{discuss}) to provide insights on how \projname{} can be used for other robot applications. Specifically, we believe that robot motion planning requires thorough scene geometry understanding. In the future, we hope to explore the capabilities of the environment encoder of \projname{} for single-view scene geometry understanding and investigate its applicability in other robotic domains.\\

\noindent \textbf{[\rvth{}] Limited reproducibility of \projname{} due to the computationally expensive training.}\\
We acknowledge that the training of \projname{} is computationally expensive and we will release the model checkpoint for public use. In the future, we hope we can generalize \projname{} on different robots and release the corresponding checkpoints.\\

\noindent \textbf{[\rvth{}] What is the trade-off of T w.r.t. to learning time, inference time, and solution quality?}\\
We observed that reducing T from 32 to lower values can result in poor solution quality in obstacle rich environments as there are insufficient number of optimization waypoints to move around obstacles. Increasing T beyond 32 make the solver take more iterations to converge as we are increasing the number of optimization variables. The increase in number of waypoints will also increase the learning time and inference time as now the network has to predict a larger number of values. We obtained T=32 from the \curobo{} paper as they were able to solve planning problems across the evaluation dataset with T=32. \\

\noindent \textbf{[\rvth{}] In sec. V.A.1, it sounds like the approach supports multiple depth input images. In the validation, obviously only a single one is used. Clarification on ``patch".}\\
As the reviewer pointed out, \projname{} can take into multiple depth images by design but we only provide one depth image during the training and the inference time, to mimic the practical real world setup where usually only one camera is available. 
We have also added the discussion on training \projname{} with multiple camera views in the future, allowing more flexible usage of \projname{} when more camera views are available (Section~\ref{discuss}). 

\noindent ``patch" is a term used in ViT~\cite{dosovitskiy2021image} referring to the smaller images generated by splitting the full image.\\

\noindent \textbf{[\rvth{}] Report metrics on the intersection of solved instances}\\
As the two baselines \bit{} and \mpinet{} has a very low success rate of 6.0\% and 8.3\% respectively (Table~\ref{tab:depth_res}), the intersection of the solved instances would be too small to be statistically meaningful.\\

\noindent \textbf{[\rvth{}] Clarifications on camera position, network dimensions and inference time. }\\
We added the clarifications in Section~\ref{sec:ps}, Section~\ref{sss:cnpm} and Section~\ref{ssec:infer}.\\


\twocolumn
\newpage





